Attentive Semantic Alignment with Offset-Aware Correlation Kernels

Semantic correspondence is the problem of establishing correspondences across images depicting different instances of the same object or scene class. One of recent approaches to this problem is to estimate parameters of a global transformation model that densely aligns one image to the other. Since an entire correlation map between all feature pairs across images is typically used to predict such a global transformation, noisy features from different backgrounds, clutter, and occlusion distract the predictor from correct estimation of the alignment. This is a challenging issue, in particular, in the problem of semantic correspondence where a large degree of image variations is often involved. In this paper, we introduce an attentive semantic alignment method that focuses on reliable correlations, filtering out distractors. For effective attention, we also propose an offset-aware correlation kernel that learns to capture translation-invariant local transformations in computing correlation values over spatial locations. Experiments demonstrate the effectiveness of the attentive model and offset-aware kernel, and the proposed model combining both techniques achieves the state-of-the-art performance.

==> ECCV 2018 (SA) Camera Ready/sections/abstract.tex <==
% !TEX root = ../main.tex

\begin{abstract}

Semantic correspondence is the problem of establishing correspondences across images depicting different instances of the same object or scene class. 
One of recent approaches to this problem is to estimate parameters of a global transformation model that densely aligns one image to the other. Since an entire correlation map between all feature pairs across images is typically used to predict such a global transformation, noisy features from different backgrounds, clutter, and occlusion distract the predictor from correct estimation of the alignment. This is a challenging issue, in particular, in the problem of semantic correspondence where a large degree of image variations is often involved. 
In this paper, we introduce an attentive semantic alignment method that focuses on reliable correlations, filtering out distractors.
For effective attention, we also propose an offset-aware correlation kernel that learns to capture translation-invariant local transformations in computing correlation values over spatial locations.
Experiments demonstrate the effectiveness of the attentive model and offset-aware kernel, and the proposed model combining both techniques achieves the state-of-the-art performance.

% -- old version
%Semantic alignment is the task of predicting the correspondences between two objects with the same class label in source and target images.






% Recent work \bhhan{often tackles this problem using \sout{has proposed semantic alignment by}} global transformation estimation in which the model predicts a set of transformation parameters to align dense points between source and target images.
%A correlation map that stores correlations of all feature pairs \bhhan{across images} is used to estimate the global transformation.
%However, noisy correlations computed from the regions with background clutters and occlusions may distract correct estimation of models.
%We propose an attentive semantic alignment algorithm that pays more attention to reliable correlations and filters out distractors for robust estimation.
%The attention process computes a single attended feature vector by weighted-averaging features using attention probabilities and the model estimates the final transformation from the attended feature vector.
%Estimating the global transformation from a set of correlations using the attention process, it is straightforward to appropriately order the correlations to capture local transformations at each spatial location .

%Therefore, we also propose offset-aware correlation kernels that are applied to correlations reordered by the offsets between features.

%A set of experiments are conducted to investigate the effectiveness of the attentive process and the OBC kernels and the proposed model utilizing both techniques achieves the state-of-the-art performance.
%The proposed method achieves the state-of-the-art performance on object geometric matching tasks on multiple benchmark datasets in both unsupervised and semi-supervised settings. 

%Image geolocalization is the task of determining where a photo was taken based only on its visual information. This task is inherently challenging since many photos have only few, possibly ambiguous, cues to their geolocation.
%Recent work has cast this task as a classification problem by partitioning the earth into a set of discrete cells that correspond to the output classes.
%The granularity of this partitioning presents a critical trade-off; using fewer, larger cells results in lower location accuracy while using more, smaller cells reduces the number of training examples per class and increases model size, making the model prone to overfitting.
%
%To tackle this issue, we propose a combinatorial partitioning algorithm, which is a simple method to generate a large number of fine-grained output classes by intersecting multiple coarse-grained partitionings of the earth.
%
%Each classifier votes for the fine-grained classes that overlap with their respective coarse-grained ones. 
%This technique allows to predict locations at a fine scale while keeping enough training examples per class.
%
%Our algorithm achieves the state-of-the-art performance in location recognition on two benchmark datasets.
%
\keywords{Semantic correspondence, attention process, offset-aware correlation kernels, attentive semantic alignment, local transformation}
\end{abstract}

==> ECCV 2018 (SA) Camera Ready/sections/attention.tex <==
% !TEX root = ../nips_2017.tex

%%%%%%%%% BODY TEXT


\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/attention.pdf}
    \caption{
    Illustration of attention process. 
    Noisy features in local transformation feature map are filtered by assigning lower probabilities to these locations.
    Arrows in boxes of local transformation feature map demonstrate features encoding local transformations, and grayscale colors in attention distribution represent magnitudes of probabilities where brighter colors mean higher probabilities.}
    \label{fig:att}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi


\section{Attentive Semantic Alignment}
\label{sec:attentive_matching}
We propose an attentive semantic alignment algorithm based on spatial attention.
To this end, we estimate a global transformation between two images, which is given by a linear combination of local transformations.
This section describes how the global transformation is obtained from local transformations by exploiting an attention model while we reserve detailed discussion about the local transformation to Section~\ref{sec:offset_kernels}.
%The local transformations are obtained by computing feature correlation between all pairs of locations in the feature maps extracted from two images. 

%facilitates attention process and focus on reliable local features only. 
%We estimate global transformation by extracting an attended feature and filtering distractors out.
%as illustrated in Fig.~\ref{fig:att}.
%While the matching task involves two input images, 
%The attention process in our model takes a local transformation feature map summarizing the feature relationships between two images, which is described in more details in Section~\ref{sec:offset_kernels}.

%In this section, we first present the overall estimation procedure with the attentive process given a feature map of local transformations, whose construction will be described in Section~\ref{sec:offset_kernels}.

\subsection{Spatial Attention on Local Transformation Features}
\label{sub:att}
Suppose that we have a local transformation feature map $\mathcal{F} \in \mathbbm{R}^{\hat{D}\times\hat{H}\times\hat{W}}$ with $\hat{H}\times\hat{W}$ spatial resolution;
each feature vector $t_{i,j}\in \mathbbm{R}^{\hat{D}}$ encodes the transformation of a local region at $(i,j)$ from a source image to a target image.
Although a feature map $\mathcal{F}$ gives sufficient information to predict the global transformation from a source to a target, local transformation features extracted from a real image pair is noisy due to various reasons such as background clutter and intra-class variations.
Therefore, we propose a model that suppresses unreliable features by the attention process and extracts an attended feature vector that summarizes local transformations from all reliable locations to estimate a accurate global transformation.
In other words, the model computes an attended transformation feature $\tau^\mathrm{att}$ by
%
\begin{align}
    \tau^\mathrm{att} %= %\sum_{i=1}^{\hat{H}}{\sum_{j=1}^{\hat{W}}{\alpha_{i,j}\tau_{i, j}}} 
    = \sum_{i=1}^{\hat{H}}{\sum_{j=1}^{\hat{W}}{\alpha_{i,j}G(t_{i, j})}}
\label{eq:attention}
\end{align}
%
where $G:\mathbbm{R}^{\hat{D}}\rightarrow \mathbbm{R}^{D'}$ is a projection function of $t_{i,j}$ into a $D'$ dimensional vector space and $\bm{\alpha} = \{\alpha_{i,j}\}$ is an attention probability distribution over feature map.
The model computes the attention probabilities by
%
\begin{equation}
    \alpha_{i,j} = \frac{\exp\left({S(t_{i,j})}\right)}{\sum_{k=1}^{\hat{H}}{\sum_{l=1}^{\hat{W}}{\exp\left({S(t_{k,l})}\right)}}} \label{eq:att_prob}
\end{equation}
%
where $S:\mathbbm{R}^{\hat{D}}\rightarrow\mathbbm{R}$ is an attention score function returning a single scalar given a local transformation feature.
%According to Eq.~\eqref{eq:attention}, the contribution of each feature $t_{i,j}$ to the attended feature $\tau^\mathrm{att}$ depends on its attention probability $\alpha_{i,j}$, which is given by scoring the transformation feature $t_{i,j}$ as specified in Eq.~\eqref{eq:att_prob}.
Note that the model learns capability to rejecting noisy features by assigning low attention scores and reducing their contribution to the attended feature.

Once the attended feature $\tau^\mathrm{att}$ over all local transformations is obtained, we compute the global transformation $\theta \in \mathbbm{R}^Q$ by a simple matrix-vector multiplication as
%the model estimates parameters of the global transformation $\theta$ with a fully-connected layer by
%
\begin{equation}
    \theta = W\tau^\mathrm{att} \label{eq:prediction}
\end{equation}
%
where $W \in \mathbbm{R}^{Q\times{D'}}$ is a weight matrix for the linear projection of the attended feature $\tau^\mathrm{att}$.

In summary, we first local transformation between two images and perform a nonlinear embedding using a projection function $G(\cdot)$.
The embedded vector is weighted by spatial attention to compute an attended feature $\tau^\mathrm{att}$ as shown in Eq.~\eqref{eq:attention}.
The global transformation vector is given by a linear projection of the attended feature parametrized by a matrix as presented in Eq.~\eqref{eq:prediction}.

%\subsection{Desired Properties of Local Transformation Features}


==> ECCV 2018 (SA) Camera Ready/sections/conclusion.tex <==
% !TEX root = ../nips_2017.tex

%%%%%%%%% BODY TEXT
\section{Conclusion}
\label{sec:conclusion}

We propose a novel approach for semantic alignment.
Our model facilitates an attention process to estimate global transformation from reliable local transformation features by suppressing distracting features.
We also propose offset-aware correlation kernels that reorder correlations of feature pairs and produce a dense feature representation of local transformations.
The experimental results show the attentive model with the proposed kernels achieves the state-of-the-art performances with large margins over previous methods on the PF-WILLOW and PF-PASCAL benchmarks.


==> ECCV 2018 (SA) Camera Ready/sections/experiments.tex <==
% !TEX root = ../main.tex

%%%%%%%%% BODY TEXT
\section{Experiments}
\label{sec:exp}

We evaluate the proposed method on public benchmarks for semantic correspondence estimation.
The experiments demonstrate that the proposed attentive method and OAC kernels are effective in semantic alignment, substantially improving the baseline models.
The codes are publicly released at \url{http://cvlab.postech.ac.kr/research/A2Net/}.


\subsection{Experimental settings}

\subsubsection{Training with self-supervision}
While the loss function requires the full supervision of $\theta_\mathrm{GT}$, it is very expensive or even impractical to collect exact ground-truth transformation parameters for non-rigid objects involving intra-class variations.
Therefore, it is hard to scale up to numerous instances and classes, restricting generalization.
For example, the largest annotation dataset at this time, PF-PASCAL, only contains total 1,351 image pairs from 20 classes, and furthermore their dense annotations are extrapolated from sparse keypoints, thus being not fully exact.
%\sout{For this reason, there is no public datasets of image pairs properly annotated with ground-truth transformation parameters for training our network.}
To work around this problem, we adopt the self-supervised learning for semantic alignment, which is free from the burden of any manual annotation, is an appealing alternative introduced in \cite{rocco2017convolutional}.
In this framework, given a public image dataset $\mathcal{D}$ without any annotations, we synthetically generate a training example $(I_\mathrm{src}, I_\mathrm{trg})$ by randomly sampling an image $I_{src}$ from $\mathcal{D}$ and computing a transformed image $I_{trg}$ by applying a random transformation $\theta_\mathrm{GT}$.
We also use mirror padding and center cropping following \cite{rocco2017convolutional} to avoid border artifacts.
The synthetic image pairs generated by this process are annotated with the ground-truth transformation parameters $\theta_\mathrm{GT}$ allowing us to train the network with full supervision.
Note that, however, this training scheme can be considered unsupervised since no annotated real dataset is used during training.

%training dataset
For the synthetic dataset generation, we use PASCAL VOC 2011~\cite{pascal-voc-2011}, and build two variations of training datasets with either affine or TPS transformation each for its corresponding network.
A set of PASCAL VOC images is kept separate to generate another set of synthetic examples for validation and the best performing models on the validation set is evaluated.


\subsubsection{Evaluation}
% evaluation datasets and evaluation metrics
Two public benchmarks called PF-WILLOW and PF-PASCAL~\cite{ham2016proposal} are used for the evaluation.
PF-WILLOW consists of about $900$ image pairs generated from $100$ images of 5 object classes. PF-PASCAL contains 1351 image pairs of 20 object classes.
%PF-PASCAL is generated from PASCAL keypoint annotation~\cite{bourdev2009poselets}. % and is more challenging than PF-WILLOW~\cite{ham2016proposal}.
Each image pair in both datasets contains different instances of the same object class such as ducks and motorbikes, \eg, left two images in Fig.~\ref{fig:geo_matching}.
The objects in these datasets have large intra-class variations and many background clutters making the task more challenging.
The image pairs of both PF-WILLOW and PF-PASCAL are annotated with sparse key points that establishe correspondences between two images.
Following the standard evaluation metric, the probability of correct keypoint (PCK)~\cite{yang2013articulated} of these benchmarks, our goal is to correctly transform the key points in the source image to their corresponding ones in the target image.
A transformed source key point is considered correct if its distance to its corresponding target key point is less than $\alpha\cdot\mathrm{max}(h, w)$, where $\alpha=0.1$, and $h$ and $w$ are height and width of the object bounding box.
Formally, PCK of a proposed model $\mathcal{M}$ is measured by
\begin{equation}
    \mathrm{PCK}(\mathcal{M})= \frac{\sum\limits_{i=1}^{N}\sum\limits_{(p_\mathrm{s}, p_\mathrm{t})\in \mathcal{P}_i}\mathbb{1}\left[d\left(\mathcal{T}_{\theta_i}\left(p_\mathrm{s}\right), p_\mathrm{t}\right) < \alpha\cdot \mathrm{max}(h, w)\right]}{\sum\limits_{i=1}^{N}{|\mathcal{P}_i|}},
\end{equation}
where $N$ is the total number of image pairs, $\mathcal{P}_i$ is a set of source and target key point pairs $(p_\mathrm{s},p_\mathrm{t})$ for $i$\superscript{th} example, $\theta_i$ is predicted transformation, and $\mathbb{1}$ is the indicator function which returns $1$ if the expression inside brackets is true and $0$ otherwise.
%Although there are public splits in PF-PASCAL, we use the entire set for the evaluation since the network is trained in an unsupervised setting.

We evaluate three different versions of the proposed model as in~\cite{rocco2017convolutional}.
The first two versions are the models with different transformations: affine and TPS transformations.
The other version sequentially merges these two models.
That is, the input image pair are first fed to the network with affine transformation, and the image pair transformed by its out is then fed to the network with TPS transformation.

% Caltech-101~\cite{fei2006one} contains 1,515 image pairs comprised of 15 pairs for all 101 object classes.
% Instead of key points, image pairs in Caltech-101 are annotated with object segmentation masks.
% We thus evaluate the proposed model based on the masks following \cite{kim2013deformable} and measure label transfer accuracy (LT-ACC), intersection-over-union (IoU), and localization error (LOC-ERR) from the transformed source mask by the model and the target mask.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
% \caption{
% Experimental results on PF-WILLOW and PF-PASCAL. 
% PCK is measured with $\alpha=0.1$.
% Scores for other models are brought from~\cite{ham2016proposal,rocco2017convolutional,han2017scnet} while scores marked with an asterisk (*) are drawn from the reproduced models by released official codes.
% The PCK scores marked with {a dagger ($^\dagger$)} are measured with height and width of the image size instead of the bounding box size.
% Note that the PCK measure with the bounding box size is more conservative than the one with the image size resulting in lower scores. 
% {PCK scores of A2Net on PF-PASCAL measured by image sizes are 0.59 (affine), 0.65 (affine+TPS) and 0.71 (affine+TPS; ResNet101). }
% }
\caption{
Experimental results on PF-WILLOW and PF-PASCAL. 
PCK is measured with $\alpha=0.1$.
Scores for other models are brought from~\cite{ham2016proposal,rocco2017convolutional,han2017scnet} while scores marked with an asterisk (*) are drawn from the reproduced models by released official codes.
The PCK scores marked with a dagger ($^\dagger$) are borrowed from~\cite{han2017scnet} measuring them with respect to the entire image size instead of the bounding box size.
Note that the PCK score with respect to the bounding box size is more conservative than the one with respect to the image size, resulting in lower scores. For example, PCK scores of A2Net on PF-PASCAL measured by image sizes are 0.59 (affine), 0.65 (affine+TPS) and 0.71 (affine+TPS; ResNet101). \\ 
}


\label{tab:main_results}
\begin{tabular}{
@{}C{0.6cm}@{}|@{}C{0.3cm}@{}@{}p{5.5cm}@{}|@{}C{2.3cm}@{}|@{}C{2.3cm}@{}
}
&&\multirow{2}{*}{Models}                             & \multicolumn{2}{c}{PCK ($\alpha=0.1$)}      \\
&&                                                    & PF-WILLOW    & PF-PASCAL     \\ \hline\hline
%&Identity (lower bound)                              & 0.19         & ----          \\ \hline
\multirow{7}{*}{\rb{Hand-crafted~}}&&DeepFlow~\cite{revaud2016deepmatching}              & 0.20         & 0.21          \\
&&GMK~\cite{duchenne2011graph}                        & 0.27         & 0.27          \\
&&SIFTFlow~\cite{liu2016sift}                         & 0.38         & 0.33          \\
&&DSP~\cite{kim2013deformable}                        & 0.29         & 0.30          \\
&&ProposalFlow (NAM)~\cite{ham2016proposal}           & 0.53         &  --           \\
&&ProposalFlow (PHM)~\cite{ham2016proposal}           & 0.55         &  --           \\
&&ProposalFlow (LOM)~\cite{ham2016proposal}           & 0.56         & 0.45          \\ \hline
\multirow{4}{*}{\rb{Self Sup.~~~}}&&GeoCNN (affine)~\cite{rocco2017convolutional}       & 0.49         & 0.39*         \\
%&GeoCNN (tps)~\cite{rocco2017convolutional}*        & 0.55          & \bf{0.81}         & 0.54          & \bf{0.24}     \\
&&GeoCNN (affine+TPS)~\cite{rocco2017convolutional}   & 0.56         & 0.50*         \\
%&&GeoCNN (affine+TPS; Res)~\cite{rocco2017convolutional}   & 0.66*         & 0.67*    \\
&&A2Net (affine)                                       & 0.52         & 0.46          \\
%&Ours (tps)                                         & 0.57          & \bf{0.81}         & 0.54          & \bf{0.24}     \\
&&A2Net (affine+TPS)                                   & 0.63    & 0.54     \\ 
&&\bf{A2Net (affine+TPS; ResNet101)}                   & \bf{0.68}    & \bf{0.59}     \\ \hline
\multirow{5}{*}{\rb{{Supervised}~}}&&UCN~\cite{choy2016universal}                        & 0.42$^\dagger$         & 0.56$^\dagger$          \\
&&FCSS~\cite{kim2017fcss}                             & 0.58        & --          \\
&&SCNet-A~\cite{han2017scnet}                         & 0.73$^\dagger$         & 0.66$^\dagger$          \\ 
&&SCNet-AG~\cite{han2017scnet}                        & 0.72$^\dagger$         & 0.70$^\dagger$          \\ 
&&SCNet-AG+~\cite{han2017scnet}                       & 0.70$^\dagger$         & 0.72$^\dagger$          \\ 
\hline
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \centering
% \caption{
% Experimental results on PF-PASCAL. 
% PCK in PF-PASCAL is measured with $\alpha=0.1$. 
% }
% \label{tab:unsup_results}
% \begin{tabular}{
% @{}C{0.1cm}@{}
% @{}p{4.2cm}@{}|@{}C{2cm}@{}|@{}C{1.9cm}@{}@{}C{1.9cm}@{}@{}C{1.9cm}@{}
% }
% &\multirow{2}{*}{Models}                             & PF-PASCAL     & \multicolumn{3}{c}{Caltech-101}	\\ 
% &                                                    & PCK           & LT-ACC            & IoU           & LOC-ERR       \\\hline\hline
% &DeepFlow~\cite{revaud2016deepmatching}              & 0.20          & 0.74	            & 0.40	        & 0.34          \\
% &GMK~\cite{duchenne2011graph}                        & 0.27          & 0.77              & 0.42          & 0.34          \\
% &SIFTFlow~\cite{liu2016sift}                         & 0.38          & 0.75              & 0.48          & 0.32          \\
% &DSP~\cite{kim2013deformable}                        & 0.29          & 0.77              & 0.47          & 0.35          \\
% &ProposalFlow (NAM)~\cite{ham2016proposal}           & 0.53          & 0.70              & 0.44          & 0.39          \\
% &ProposalFlow (PHM)~\cite{ham2016proposal}           & 0.55          & 0.75              & 0.48          & 0.31          \\
% &ProposalFlow (LOM)~\cite{ham2016proposal}           & 0.56          & 0.78              & 0.50          & 0.26          \\ \hline
% &GeoCNN (affine)~\cite{rocco2017convolutional}       & 0.49          & 0.76 (0.79)       & 0.52 (0.51)   & 0.27 (0.25)   \\
% %&GeoCNN (tps)~\cite{rocco2017convolutional}*         & 0.55          & \bf{0.81}         & 0.54          & \bf{0.24}     \\
% &GeoCNN (affine+tps)~\cite{rocco2017convolutional}   & 0.56          & {\bf0.81} (0.82)  & 0.56 (0.56)   & 0.27 (0.25)   \\
% &Ours (affine)                                       & 0.52          & 0.78              & 0.53          & 0.26          \\
% %&Ours (tps)                                          & 0.57          & \bf{0.81}         & 0.54          & \bf{0.24}     \\
% &Ours (affine+tps)                                   & 0.63          & \bf{0.81}         & \bf{0.58}     & 0.27          \\
% \hline
% \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Results}
\subsubsection{Comparisons to other models} 
Table~\ref{tab:main_results} shows the comparative results on both PF-WILLOW and PF-PASCAL benchmarks.
It includes (i) previous methods using hand-crafted features: DeepFlow~\cite{revaud2016deepmatching}, GMK~\cite{duchenne2011graph}, SIFTFlow~\cite{liu2016sift}, DSP~\cite{kim2013deformable}, and ProposalFlow~\cite{ham2016proposal}, (ii) self-supervised alignment methods: GeoCNN~\cite{rocco2017convolutional} and the proposed attentive alignment network (A2Net),  (iii) supervised methods: UCN~\cite{choy2016universal}, FCSS~\cite{kim2017fcss}, and SCNet~\cite{han2017scnet}. 
%, we show the lower bound (Identity) by measuring PCK with the identity transformation by which the original key point locations in the source image are preserved in the target image.
Note that the supervised methods are trained with either a weakly or strongly annotated data and that many of their PCKs are measured under a different criterion that are not directly comparable to the other scores. 
By contrast, our method is only trained using synthetic data with self-supervision.
As shown in Table~\ref{tab:main_results}, the proposed method substantially outperforms all the other methods that are directly comparable. %except SCNet models that are supervised using PF-PASCAL dataset in learning. 
Using VGG-16 feature extractor, the proposed method improves 12.5 \% and {8} \% of PCK over the non-attentive alignment method~\cite{rocco2017convolutional} on PF-WILLOW and PF-PASCAL, respectively.
This reveals the effect of the proposed attention model for semantic alignment. 
The quality of the model is further improved when incorporated with a more advanced feature extractor such as ResNet101.
%It is also notable that our model with affine transformation already performs similarly to the  performances drawn by ProposalFlow and GeoCNN.
It is notable that the proposed model outperforms some of supervised methods, UCN~\cite{choy2016universal} and FCSS~\cite{kim2017fcss}, while it is trained without any real datasets.

% \jmlee{and ResNet-101~\cite{He2015resnet}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{
PCKs of ablations on PF-WILLOW trained with PASCAL VOC 2011. 
Scores of GeoCNN are obtained from the code released by the authors.
The numbers of network parameters exclude the feature extractors since all models share the same feature extractor.
}
\label{tab:ablation}
\begin{tabular}{
@{}C{0.2cm}@{}
@{}p{4cm}@{}|@{}C{2.4cm}@{}|@{}C{1.5cm}@{}@{}C{1.5cm}@{}@{}C{2.1cm}@{}
}
&Models                     &\# of params       & Affine    & TPS       & Affine+TPS    \\ \hline\hline
&GeoCNN~\cite{rocco2017convolutional} & 1.63M (x1.7)      & 0.430     & 0.539     & 0.560         \\
&GeoCNN+Attention           & 1.41M (x1.5)      & 0.423     & 0.478     & 0.476         \\
&GeoCNN+OACK                & 1.12M (x1.2)      & 0.491     & 0.555     & 0.609         \\
&Attention+OACK (A2Net)      & \bf{0.95M (x1.0)} & \bf{0.521}& \bf{0.563}& \bf{0.626}    \\
\hline
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{PCKs of affine models on PF-WILLOW with different training datasets: PASCAL VOC 2011 and Tokyo Time Machine. Scores for GeoCNN are brought from \cite{rocco2017convolutional}.}
\label{tab:generalization}
\begin{tabular}{
@{}C{0.2cm}@{}
@{}p{2.2cm}@{}|@{}C{3.2cm}@{}|@{}C{3.2cm}@{}
}
&Models                     & PASCAL VOC 2011   & Tokyo Time Machine    \\ \hline\hline
&GeoCNN~\cite{rocco2017convolutional} & 0.45              & 0.49                  \\
&A2Net                       & \bf{0.52}         & \bf{0.51}             \\
\hline
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Ablation study}

As our proposed model combines two distinct techniques we perform ablation studies to demonstrate their effects.
We mainly compare the proposed model to GeoCNN as it directly predicts the global transformation parameters using the correlation layer.
To see the effect of the proposed OAC kernels, we build a model, referred to as GeoCNN+OACK, by replacing the correlation layer of GeoCNN with the OAC kernels.
As shown in Tabel~\ref{tab:ablation}, the use of the OAC kernels already improves the performances of GeoCNN for all three versions.
Moreover, the OAC kernels reduce the number of parameters in the network since it uses dense representations of local transformations allowing channel compression.
Applying attention process on top of correlation layer (GeoCNN+Attention) drops the performance.
This is because the correlation map does not encode local transformations in a translation invariant representations.
On the other hand, the attention process with the OAC kernels, which is the proposed model, further improves the performances as the distracting regions can be suppressed during the transformation estimation thanks to the local transformation feature map obtained by the OAC kernels.
It is also notable that applying the attention process reduces the number of model parameters because the model does not need extra layers that combine all local information to produce the global estimation; instead, the models simply aggregate local features with attention distribution.
This additional parameter reduction results in 70 \% fewer parameters than GeoCNN while the models maintain superior performance improvements.





\subsubsection{Sensitivity to training datasets}
While both our model and GeoCNN are generally applicable to any image datasets, we experiment the sensitivity of the models to changing training datasets.
We train both models with the affine transformation on another image dataset, called Tokyo Time Machine~\cite{arandjelovic2016netvlad}, using the same synthetic generation process, and show how much the performances change depending on the datasets.
Table~\ref{tab:generalization} shows that the proposed model is less dependent on the choice of the training dataset compared to GeoCNN.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/qualitative.pdf}
    \caption{
    Qualitative results of the attentive semantic alignment.
    Each row shows an example of PF-PASCAL benchmark.
    Given the source and target images shown in first and third columns, we visualize the attention maps of the affine model (second column), the transformed image by the affine model (fourth column) and the final transformed image by the affine+TPS model (last column).
    Since the models learn inverse transformation, the target image is transformed toward the source image while the attention distribution is drawn over the source image.
    The model attends to the objects to match and estimates dense correspondences despite intra-class variations and background clutters.
    }
    \label{fig:qualitative}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Qualitative results with attention visualizations}
Fig.~\ref{fig:qualitative} presents some qualitative examples of our model on PF-PASCAL.
In our experimental setting, the models learn to predict inverse transformation.
Therefore, we transform the target image toward the source image using the estimated inverse transformation whereas the attention distribution is drawn over the source image.
The proposed model attends to the target objects with other regions suppressed and predicts the global transformation based on reliable local features.
The model estimates the transformation despite large intra-class variations such as an adult vs. a kid.

We also investigate some failure cases of the proposed model in Fig.~\ref{fig:failure}.
The model is confused when there are multiple objects of the same class in an image or have a large obstacles occluding the matching objects.
Also, objects in some examples are hard to visually recognize and lead mismatches.
For instance, the model fails to correctly match a wooden chair to a transparent chair although the model attends to the correct region in the second example of Fig.~\ref{fig:failure}.
It is challenging even for human to recognize the transparent chair and its corresponding key points.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/failure_cases.pdf}
    \caption{
    Some failure cases of the proposed model with the affine transformation.
    Each row shows an example of PF-PASCAL.
    Each example contains 1) source image, 2) source image masked by attention distribution, 3) target image and 4) target image transformed by the predicted affine parameters.
    Even though the model attends to the matching objects, the model fails to find the correct correspondences due to multiple objects of the same class causing ambiguity or hard examples that are difficult to visually percept.
    }
    \label{fig:failure}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> ECCV 2018 (SA) Camera Ready/sections/introduction.tex <==
% !TEX root = ../main.tex

%%%%%%%%% BODY TEXT
\section{Introduction}
\label{sec:introduction}

% Geometric matching and traditional approaches
Semantic correspodence is the problem of establishing correspondences across images depicting different instances
of the same object or scene class. %~\cite{forsyth2002computer,hartley2003multiple}
Compared to conventional correspondence tasks handling pictures of the same scene, such as stereo matching~\cite{hosni2013fast,okutomi1993multiple} and motion estimation~\cite{dosovitskiy2015flownet,weinzaepfel2013deepflow,revaud2016deepmatching}, 
  the problem of semantic correspondence involves substantially larger changes in appearance and spatial layout, thus remaining very challenging.
%image stitching~\cite{szeliski2006image}, image enhancement~\cite{hacohen2011non}, 3D reconstruction~\cite{hartley2003multiple,agarwal2011building}, semantic segmentation~\cite{rubinstein2013unsupervised} and motion estimation~\cite{dosovitskiy2015flownet,weinzaepfel2013deepflow}.
For this reason, traditional approaches based on hand-crafted features such as SIFT~\cite{lowe2004distinctive,liu2016sift} and HOG~\cite{dalal2005histograms,ham2016proposal,taniai2016joint} 
%using a geometric model like epipolar geometry.
%While these approaches achieve reasonable performances especially \bhhan{by incorporating} pruning techniques for incorrect matches~\cite{schmid1997local,sivic2003video,fischler1987random,leibe2008robust}, they 
do not produce satisfactory results on this problem due to lack of high-level semantics in local feature representations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/geo_matching.pdf}
    \caption{
    The proposed attentive semantic alignment. 
    Our model estimates dense correspondences of objects by predicting a set of global transformation parameters via an attention process. The attention process spatially focuses on the reliable local transformation features, filtering out irrelevant backgrounds and clutter. 
    }
    \label{fig:geo_matching}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

While previous approaches to the problem focus on introducing an effective spatial regularizer in matching~\cite{liu2016sift,kim2013deformable,ham2016proposal},  
%With the remarkable success of deep learning approaches in visual recognition,
%several learning-based methods have also been proposed for
% improvement by deep networks and the correlation layer
recent convolutional neural networks have advanced this area 
%and the current top-performing methods~\cite{rocco2017convolutional,han2017scnet} 
by learning high-level semantic features~\cite{choy2016universal,rocco2017convolutional,han2017scnet,ufer2017deep,kim2017dctm,kim2017fcss,novotny2017anchornet}.
One of the main approaches~\cite{rocco2017convolutional} is to estimate parameters of a global transformation model that densely aligns one image to the other. % as shown in Fig.~\ref{fig:geo_matching}. 
In contrast to other approaches, it casts the whole correspondence problem for all individual features into a simple regression problem with a global transformation model, thus predicting dense correspondences through the efficient pipeline. 
On the other hand, however, the global alignment approach may be easily distracted; 
An entire correlation map between all feature pairs across images is used to predict such a global transformation, and thus noisy features from different backgrounds, clutter, and occlusion, may distract the predictor from correct estimation of the alignment. This is a challenging issue, in particular, in the problem of semantic correspondence where a large degree of image variations is often involved. 

In this paper, we introduce an attentive semantic alignment method that focuses on reliable correlations, filtering out distractors as shown in Fig.~\ref{fig:geo_matching}.
%The attention process takes input features and transform them into a single attended feature vector by predicting attention probabilities.
For effective attention, we also propose an offset-aware correlation kernel that learns to capture translation-invariant local transformations in computing correlation values over spatial locations.
%are applied to correlations reordered by the offsets between features.
%estimating the global transformation from a set of correlations using the attention process, it is straightforward to appropriately order the correlations to capture local transformations at each spatial location .
%Since the final transformation is predicted on the attended feature vector, which is a linear sum of local features, each local feature should convey cues for the global transformation estimation.
%\hsseo{Since the attention process estimates the global transformation from averaged local features with attention distribution as weights, we introduce offset-based correlation (OBC) kernels that can capture local transformation by reordering correlations based on the offsets of the features.}
%Unlike the previous correlation layer, the proposed correlation kernels have capability of capturing local transformations by sharing kernel weights based on the relative offsets between features.
%
%The proposed method achieves the state-of-the-art performance on object geometric matching tasks on multiple benchmark datasets in both unsupervised and semi-supervised settings. 
%Also, original feature locations for each correlation are not encoded within correlation values.
%Second, the feature locations are not properly encoded to compute local transformations from the feature correlation tensor.
%{\color{blue}Therefore, it is critical to use the indices of the correlation map for the transformation estimation, which is why the entire correlation map is used for the transformation estimation in~\cite{rocco2017convolutional}.}
%To overcome these limitations, we propose a novel semantic alignment network using an attention process and offset-aware correlation (OAC) kernels.
%The attention process allows our model to focus on object-related regions while maintaining the quality of the global transformation estimation.
%The proposed model predicts a spatial attention distribution over a feature map encoding local transformations at each spatial location, and obtains an attended feature vector by aggregating the local transformation feature at every location weighted by its attention probability.
%Through this process, the model filters out distracting regions by assigning low probabilities \bhhan{to them.}
%To overcome this limitation and make the model estimate the global transformation parameters while still focusing on object-related regions, we introduce an attention process~\cite{} that efficiently rejects irrelevant features.
%To successfully utilize the attention process, we adapt a local transformation feature map that is obtained by OAC kernels replacing the correlation map of the correlation layer.
%\bhhan{To take advantage of the attention process, we replace the correlation map given by the correlation layer with a local transformation feature map obtained by applying OAC kernels.}
The resultant feature map of offset-aware correlation (OAC) kernels is computed from two input features, where each activation of the feature map represents how smoothly a source feature is transformed spatially to the target feature map. This use of OAC kernels greatly improves a subsequent attention process. 
%The OAC kernels encode local transformations in the feature maps \bhhan{by implicitly constructing a reordered correlation map using the offsets with respect to relative locations between the source and target features.}
Experiments demonstrate the effectiveness of the attentive model and offset-aware kernel, and the proposed model combining both techniques achieves the state-of-the-art performance.


Our contribution in this work is threefold:
\begin{itemize}
    \item[$\bullet$] The proposed algorithm incorporates an attention process to estimate a global transformation from a set of inconsistent and noisy local transformations for semantic image alignment.
    %To the best of our knowledge, our method is the first semantic alignment method applying an attention process.
    %\item The proposed kernels represent local transformations as dense features reducing the number of dimensions required and consequently the number of parameters in the following layer.
    \item[$\bullet$] We introduce offset-aware correlation kernels to guide the network in capturing local transformations at each spatial location effectively, and employ the kernels to compute feature correlations between two images for better representation of semantic alignment.
    \item[$\bullet$] The proposed network with the attention module and offset-aware correlation kernels achieves the state-of-the-art performances on semantic correspondence benchmarks.
\end{itemize}

The rest of the paper is organized as follows. 
We overview the related work in Section~\ref{sec:rel_work}.
Section~\ref{sec:net_arch} describes our proposed network with the attention process and the offset-based correlation kernels.
%Section~\ref{sec:attentive_matching} and \ref{sec:offset_kernels} describe the attentive semantic alignment and the offset-based correlation kernels, respectively.
%Then, our deep neural network for semantic alignment is explained in Section~\ref{sec:net_arch}.
Finally, we show the experimental results of our method and conclude the paper in Section~\ref{sec:exp} and \ref{sec:conclusion}.

==> ECCV 2018 (SA) Camera Ready/sections/net_arch.tex <==
% !TEX root = ../main.tex

\section{Deep Attentive Semantic Alignment Network}
\label{sec:net_arch}

We propose a deep neural network architecture for semantic alignment incorporating an attention process with a novel offset-aware correlation kernel.
Our network takes as inputs two images and estimates a set of global transformation parameters using three main components: feature extractor, local transformation encoder, and attentive global transformation estimator as presented in Fig.~\ref{fig:net_arch}.
We describe each of these components in details.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/net_arch.pdf}
\caption{
Overall architecture of the proposed network.
It consists of three main components: feature extractor, local transformation encoder, and attentive global transformation estimator. For details, see text. 
}
\label{fig:net_arch}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse
We build a deep neural network for semantic alignment facilitating the techniques described in Section~\ref{sec:attentive_matching} and \ref{sec:offset_kernels}.
Our network estimates a set of global transformation parameters using three main components: feature extractor, local transformation encoder and attentive global transformation estimator as presented in Fig.~\ref{fig:net_arch}.
We describe the detailed architecture and training procedure for each component below.
\fi


\subsection{Feature extractor}
Given source and target images, we first extract their image feature maps $\bm{f}^\mathrm{src},\bm{f}^\mathrm{trg} \in \mathbbm{R}^{D\times H\times W}$ using a fully convolutional image feature extractor, where $H$ and $W$ are height and width of input images, respectively.
%Each feature map consists of $H\times W$ features and a feature at each spatial location embeds a local image patch in a dense grid.
We use a VGG-16~\cite{simonyan2015very} model pretrained on ImageNet~\cite{deng2009imagenet} and extract features from its \texttt{pool4} layer.
We share the weights of the feature extractor for both source and target images.
Input images are resized into $240\times240$ and fed to the feature extractor resulting in $15\times15$ feature maps with $512$ channels.
After extracting the features, we normalize them using $L_2$ norm.

\subsection{Local transformation encoder}
Given source and target feature maps from the feature extractor, the model encodes local transformations of the source features with respect to the target feature map.
The encoding is given by introducing a novel offset-aware correlation (OAC) kernel, which facilitates to overcome limitations of conventional correlation layers~\cite{rocco2017convolutional}.
We briefly describe details of the correlation layer including its limitations and discuss the proposed OAC kernel.

\subsubsection{Correlation layer}

The correlation layer computes correlations of all pairs of features from the source and the target images~\cite{rocco2017convolutional}.
Specifically, the correlation layer takes two feature maps as its inputs and constructs a correlation map $\bm{c} \in \mathbbm{R}^{HW \times H \times W}$, which is given by
%
\begin{equation}
    c_{i,j} = {f^\mathrm{src}_{i,j}}^\top \hat{\bm{f}}^\mathrm{trg},
\end{equation}
%
where $c_{i,j} \in \bm{c}$ is a $HW$ dimensional correlation vector at a spatial location $(i, j)$, $f_{i,j}^\mathrm{src} \in \bm{f}^\mathrm{src}$ is a feature vector at a location $(i, j)$ of the source image, and $\hat{\bm{f}}^\mathrm{trg} \in \mathbbm{R}^{D\times HW}$ is a spatially flattened feature map of $\bm{f}^\mathrm{trg}$ of the target image.
In other words, each correlation vector $c_{i,j}$ consists of correlations between a single source feature $f_{i,j}^\mathrm{src}$ and all target features of $\bm{f}^\mathrm{trg}$.
Although each element of a correlation vector maintains the correspondence likelihood of a source feature onto a certain location in the target feature map, the order of elements in the correlation vector is based on the absolute coordinates of individual target features regardless of the source feature location. This means that decoding the local displacement of the source feature requires not only the vector itself but also the spatial location of the source feature.
%Note that the values in correlation vectors are arranged by the absolute ordering of the target features.
For example, consider a correlation vector $c_{i,j}=[1, 0, 0, 0]^\top$ between $2\times 2$ feature maps, each element of which is the correlation of $f^\mathrm{src}_{i,j}$ with $f^\mathrm{trg}_{0,0}$, $f^\mathrm{trg}_{0,1}$, $f^\mathrm{trg}_{1,0}$ and $f^\mathrm{trg}_{1,1}$. The displacement represented by the vector varies with the coordinate of the source feature $(i,j)$. When $(i,j)=(0,0)$, it indicates that the source feature $f^\mathrm{src}_{0,0}$ remains at the same location $(0,0)$ in the target feature map. When $(i,j)=(0,1)$, it implies that $f^\mathrm{src}_{0,1}$ is moved to the left of its original location in the target feature map.

Given a correlation map, decoding the local displacement of a source feature requires incorporating the offset information from the source feature to individual target features. And, this local process is crucial for subsequent spatial attention process in the next section. Therefore, we first introduce an offset-aware correlation kernel that utilizes the offset of features during the kernel application.

%This is especially problematic when applying the attention processes because we apply translation invariant functions, $G$ and $S$, to every local transformation feature where the feature alone should convey sufficient information for estimating the attention scores and generating feature vector for transformation estimation.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.49\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{figures/correlation_kernels_0.pdf}
\subcaption{kernel alignment for $h_{0,0}$}
\label{fig:kernels_00}
\end{subfigure}
%
\begin{subfigure}[b]{0.49\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{figures/correlation_kernels_1.pdf}
\subcaption{kernel alignment for $h_{0,1}$}
\label{fig:kernels_01}
\end{subfigure}
\caption{
Offset-aware correlation kernel at different source locations: (a) at $(0,0)$ and (b) at $(0,1)$.
Each dotted line connects source and target features to compute correlation, and $w_{i,j}$ represents a kernel weight for the dotted line.
Note that kernel weights are associated with different correlation pairs when source locations vary.
}
\label{fig:kernels}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Offset-aware correlation kernels}
Similarly to the correlation layer, our OAC kernels also take two input feature maps and utilize correlations of all feature pairs between these feature maps.
The kernels naturally capture the displacement of a source feature in the target feature map by aligning kernel weights based on the offset between the source and target features for each correlation as illustrated in Fig.~\ref{fig:kernels}.
Formally speaking, an OAC kernel captures feature displacement of a source feature $f^\mathrm{src}_{i,j}$ by
%
\begin{align}
    h_{i, j}^{(n)} &=\sum_{k=1}^{H}{\sum_{l=1}^{W}{w_{i-k, j-l}^{(n)} c_{i,j;k,l}}} \\
    &=\sum_{k=1}^{H}{\sum_{l=1}^{W}{w_{i-k, j-l}^{(n)} {f^\mathrm{src}_{i,j}}^\top f^\mathrm{trg}_{k,l}}},
\end{align}
%
where $h^{(n)}_{i,j}$ is the kernel output with the kernel index $n$, $c_{i,j;k,l}$ is the correlation between a source feature $f^\mathrm{src}_{i,j}$ and a target feature $f^\mathrm{trg}_{k,l}$, and $\Phi^{(n)}= \{w^{(n)}_{s,t}\}$ is a set of the kernel weights.
Note that the kernel weights are indexed by offset between the source and target features, and shared for correlations of any feature pair with the same offset.
For example, in Fig.~\ref{fig:kernels_00}, $w_{0,0}$ is associated with the target feature at $(0,0)$ because the source location is $(0,0)$.
The same weight $w_{0,0}$ is associated with the target feature at $(0,1)$ when the source location is $(0,1)$ as in Fig.~\ref{fig:kernels_01} because the offset between these features is $(0,0)$.
Also note that each kernel output $h^{(n)}_{i,j}$ at a location $(i,j)$ captures the displacement of its corresponding source feature $f^\mathrm{src}_{i,j}$ at the same location.

While a proposed kernel captures a single aspect of feature displacement, a set of the proposed kernels produce a dense feature representation of feature displacement for each source feature.
We use $128$ OAC kernels resulting in a feature displacement map $\bm{h} \in \mathbbm{R}^{128\times15\times15}$ encoding the displacement of each source feature.
We set ReLU as the activation functions of the kernel outputs, and compute normalized correlations in OAC kernels since normalization further improves the scores as observed in \cite{rocco2017convolutional}.
%In practice, we use normalized correlations as the normalization further improves the scores as observed in \cite{rocco2017convolutional} and ReLU is set as the activation function of the kernel outputs. 

%\subsubsection{Reordering correlations and feature compression}
In practice, the proposed OAC kernels are implemented by two sub-procedures.
We first compute the normalized correlation map reordered based on the offsets between the locations of the source and target features.
In this reordered correlation map, every correlation with the same relative displacement is arranged in the same channel.
This reordering results in $(2H-1)(2W-1)$ possible offsets and thus the size of the output tensor becomes $(2H-1)(2W-1) \times H \times W$ where many of the values are zeros due to non-existing pairs for some offsets. 
%This process increase the number of channels.
Then, we use a $1\times1$ convolutional layer to compute the dense feature representation from the raw displacement information captured in the reordered correlation map.
Note that this process significantly reduces the number of channels by compactly encoding various aspects of the local displacements into dense representations.



%\jmlee{In practice, we firstly reorder the correlations of the correlation map using the offsets between source and target features instead of the absolute index of target features. That is, the correlations with the same relative displacements are arranged in the same channel of the feature map.
%This reordering results in $(2H-1)(2W-1)$ possible offsets and thus the output tensor is the size of $(2H-1)(2W-1) \times H \times W$ where many of the values are zeros due to non-existing pairs for some offsets.
%To reduce the number of channels, we apply $1\times1$ convolution operation compressing features into a dense representation.}

%\jmlee{Note that this reordering scheme injects the relative displacement information of an image feature into the correlation vector representation by arranging the dimensions. Thus, this feature displacement map abstracts raw displacement information as a dense flow. 
% Thus, this reordered correlation vector itself already contains local transformation information, and is appropriate as an input to translation invariant operations such as $G$ and $S$ in the attention process.}

\subsubsection{Encoding local transformation features}
Since the feature displacement map conveys the movement of each source feature independently, each feature alone is not sufficient to predict the global transformation parameters.
To allow the network predicts the global transformation from local features in the attention process, we construct a local transformation feature map by combining spatially adjacent feature displacement information captured by $\bm{h}$.
%Once the feature displacement map $\bm{h}$ is obtained, the proposed network then extracts local transformation features by merging spatially adjacent feature displacement information captured by $\bm{h}$.
That is, the proposed network feeds the feature displacement map $\bm{h}$ to a $7\times7$ convolution layer with $128$ output channels applied without padding.
This convolution layer results in a local transformation feature map $\mathcal{F}\in\mathbbm{R}^{128\times9\times9}$.
Note that each feature $t_{i,j} \in \mathcal{F}$ captures transformations occurred in a local region. % by merging displacements of features within the local region.
We utilize this local transformation feature map to predict the global transformation through an attention process.

%where $c_{i,j;k,l}$ is the correlation between a source feature $f^\mathrm{src}_{i,j}$ and a target feature $f^\mathrm{trg}_{k,l}$, $n$ is the kernel index, and $\Phi^{(n)}= \{w^{(n)}_{s,t}\}$ is a set of the kernel weights.
%Each spatial location of the kernel output $\bm{h} \in \mathbbm{R}^{N\times H\times W}$ corresponds to the same location of the source feature map $\bm{f}^\mathrm{src}$.
% Note that the kernel weights are indexed by the relative offset between the source and target features, and shared for the target features with the same relative offsets across all spatial locations in the source feature map.
% For example, in Fig.~\ref{fig:kernels_00}, $w_{0,0}$ is associated with the target feature at $(0,0)$ because the source location is $(0,0)$.
% Also, the same weight $w_{0,0}$ is associated with the target feature at $(0,1)$ when the source location is $(0,1)$ as in Fig.~\ref{fig:kernels_01}.





\iffalse
To overcome such limitation, we reorder the correlations of the correlation map using the offsets between source and target features instead of the absolute index of target features.
That is, the correlations with the same relative displacements are arranged in the same channel of the feature map.
This reordering results in $(2H-1)(2W-1)$ possible offsets and thus the output tensor is the size of $(2H-1)(2W-1) \times H \times W$ where many of the values are zeros due to non-existing pairs for some offsets.
To reduce the number of channels, we apply $1\times1$ convolution operation compressing features into a dense representation.

Note that this reordering scheme injects the relative displacement information of an image feature into the correlation vector representation by arranging the dimensions.
Thus, this reordered correlation vector itself already contains local transformation information, and is appropriate as an input to translation invariant operations such as $G$ and $S$ in the attention process.



We interpret the above reordering schemes with feature compression as a new type of kernels, referred to as OAC kernels, that take two image feature maps and produce a single output feature map containing local transformation features.
%
%The proposed OBC kernels takes as inputs two image feature maps extracted from the source and target images and produces a single output feature map whose feature vector at a spatial location captures the local transformation of the source feature at the same location in the target feature map.
%Local transformation encoding is achieved by using correlations of a source feature at a single location with all target features along the spatial dimensions as the proposed kernels assign weights to each of these correlations.
Note that the weights of $1\times1$ convolution layer are aligned with the reordered correlations.
That is, the weights are shared among those correlation values that are computed from the source and target features with the same offset.

%Formally speaking, let $\bm{f}^\mathrm{src}, \bm{f}^\mathrm{trg} \in \mathbbm{R}^{D\times H\times W}$ be the source and target feature maps respectively where both feature maps are extracted by the same CNN from the source and target images.
Therefore, we formally define a OAC kernel that computes a dense local transformation feature $h^{(n)}_{i,j}$ by
%
\begin{align}
    h_{i, j}^{(n)} &=\sum_{k=1}^{H}{\sum_{l=1}^{W}{w_{i-k, j-l}^{(n)} c_{i,j;k,l}}} \\
    &=\sum_{k=1}^{H}{\sum_{l=1}^{W}{w_{i-k, j-l}^{(n)} {f^\mathrm{src}_{i,j}}^\top f^\mathrm{trg}_{k,l}}}
\end{align}
%
where $c_{i,j;k,l}$ is the correlation between a source feature $f^\mathrm{src}_{i,j}$ and a target feature $f^\mathrm{trg}_{k,l}$, $n$ is the kernel index, and $\Phi^{(n)}= \{w^{(n)}_{s,t}\}$ is a set of the kernel weights.
Each spatial location of the kernel output $\bm{h} \in \mathbbm{R}^{N\times H\times W}$ corresponds to the same location of the source feature map $\bm{f}^\mathrm{src}$.
Note that the kernel weights are indexed by the relative offset between the source and target features, and shared for the target features with the same relative offsets across all spatial locations in the source feature map.
For example, in Fig.~\ref{fig:kernels_00}, $w_{0,0}$ is associated with the target feature at $(0,0)$ because the source location is $(0,0)$.
Also, the same weight $w_{0,0}$ is associated with the target feature at $(0,1)$ when the source location is $(0,1)$ as in Fig.~\ref{fig:kernels_01}.
%In consequence, two outputs of the proposed kernels $h_{i,j}, h_{k,l} \in \mathbbm{R}^{N}$ may differ even when $f_{i,j}^\mathrm{src}=f_{k,l}^\mathrm{src}$ if $(i,j)\ne (k,l)$.
%This weight sharing scheme lets the kernel output capture the spatial relationships between source and target images and encode the local transformations from the source to the target image.

This interpretation allows us to reduce the time complexity of the kernel output computation.
The reordered correlation map with a $1\times1$ convolution requires $N(2H^2-H)(2W^2-W)$ multiplications whereas only $NH^2W^2$ multiplications are required using OAC kernels.


Once the source and target feature maps are extracted by the feature extractor, a local transformation feature map is constructed from them using the OAC kernels introduced in Section~\ref{sec:offset_kernels}.
When implementing the kernels, we use normalized correlations since the normalization further improves the scores as in~\cite{rocco2017convolutional}.
Also, ReLU is set as the activation function to the kernel outputs.
We use $N=128$ OAC kernels resulting in $128\times15\times15$ tensor where each $128$ dimensional feature vector encode the local transformations of the feature at the same location in the source feature map.


The local transformations captured by the proposed kernels are about feature displacement between the source and target feature maps since the kernels take a single source feature for computing each output vector.
To enable the model to have a glimpse of the global transformation at each spatial location, we further merge the kernel outputs locally using a convolutional layer with batch normalization to obtain local transformations from larger patches.
The convolution layer is size of $7\times7$ with $128$ channels, and is applied to the feature map without padding resulting in a $128\times9\times9$ tensor, which passed to the attentive global transformation estimator after applying ReLU.

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/attention.pdf}
    \caption{
    Illustration of attention process. 
    Noisy features in local transformation feature map are filtered by assigning lower probabilities to these locations.
    Arrows in boxes of local transformation feature map demonstrate features encoding local transformations, and grayscale colors in attention distribution represent magnitudes of probabilities where brighter colors mean higher probabilities.}
    \label{fig:att}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Attentive global transformation estimator}
\label{sub:att}
After local transformation encoding, a set of global transformation parameters is estimated with an attention process.
% To this end, we estimate a global transformation between two images, which is given by a linear combination of local transformations.
% This section describes how the global transformation is obtained from local transformations by exploiting an attention model while we reserve detailed discussion about the local transformation to Section~\ref{sec:offset_kernels}.
Given a local transformation feature map $\mathcal{F}\in \mathbbm{R}^{\hat{D}\times\hat{H}\times\hat{W}}$ extracted by OAC kernels with a convolution layer, the network focuses on reliable local transformation features by filtering out distracting regions as depicted in Fig.~\ref{fig:att} to predict the parameters from the aggregation of those features. 
%each feature vector $t_{i,j}\in \mathcal{F}$ encodes the transformation of a local region at $(i,j)$ from a source image to a target image.
Although a feature map $\mathcal{F}$ gives sufficient information to predict the global transformation from source to target, local transformation features extracted from a real image pair is noisy due to image variations such as background clutter and intra-class variations.
Therefore, we propose a model that suppresses unreliable features by the attention process and extracts an attended feature vector that summarizes local transformations from all reliable locations to estimate an accurate global transformation.
In other words, the model computes an attended transformation feature $\tau^\mathrm{att}$ by
%
\begin{align}
    \tau^\mathrm{att} %= %\sum_{i=1}^{\hat{H}}{\sum_{j=1}^{\hat{W}}{\alpha_{i,j}\tau_{i, j}}} 
    = \sum_{i=1}^{\hat{H}}{\sum_{j=1}^{\hat{W}}{\alpha_{i,j}G(t_{i, j})}},
\label{eq:attention}
\end{align}
%
where $G:\mathbbm{R}^{\hat{D}}\rightarrow \mathbbm{R}^{D'}$ is a projection function of $t_{i,j}$ into a $D'$ dimensional vector space and $\bm{\alpha} = \{\alpha_{i,j}\}$ is an attention probability distribution over feature map.
The model computes the attention probabilities by
%
\begin{equation}
    \alpha_{i,j} = \frac{\exp\left({S(t_{i,j})}\right)}{\sum_{k=1}^{\hat{H}}{\sum_{l=1}^{\hat{W}}{\exp\left({S(t_{k,l})}\right)}}},\label{eq:att_prob}
\end{equation}
%
where $S:\mathbbm{R}^{\hat{D}}\rightarrow\mathbbm{R}$ is an attention score function producing a single scalar given a local transformation feature.
%According to Eq.~\eqref{eq:attention}, the contribution of each feature $t_{i,j}$ to the attended feature $\tau^\mathrm{att}$ depends on its attention probability $\alpha_{i,j}$, which is given by scoring the transformation feature $t_{i,j}$ as specified in Eq.~\eqref{eq:att_prob}.
Note that the model learns to suppress noisy features by assigning low attention scores and reducing their contribution to the attended feature.

Once the attended feature $\tau^\mathrm{att}$ over all local transformations is obtained, we compute the global transformation $\theta \in \mathbbm{R}^Q$ by a simple matrix-vector multiplication as
%the model estimates parameters of the global transformation $\theta$ with a fully-connected layer by
%
\begin{equation}
    \theta = W\tau^\mathrm{att}, \label{eq:prediction}
\end{equation}
%
where $W \in \mathbbm{R}^{Q\times{D'}}$ is a weight matrix for linear projection of the attended feature $\tau^\mathrm{att}$.

In summary, we first compute local transformation between two images and perform a nonlinear embedding using a projection function $G(\cdot)$.
The embedded vector is weighted by spatial attention to compute an attended feature $\tau^\mathrm{att}$ as shown in Eq.~\eqref{eq:attention}.
The global transformation vector is obtained by linear projection of the attended feature, which is parametrized by a matrix as presented in Eq.~\eqref{eq:prediction}.








%The output tensor of the local transformation encoder is used as the local transformation feature map $\mathcal{F}$ in Section~\ref{sub:att} where $\hat{D}=128$ and $\hat{H}=\hat{W}=9$.

We use multi-layer perceptrons (MLPs) for $G$ and $S$ in Eq.~\eqref{eq:attention} and \eqref{eq:att_prob}.
$G$ is a two-layer MLP with $128$ hidden and output ReLU activations.
Since the feature representations produced by $G$ is directly used for the final estimation as a linear mapping in Eq.~\eqref{eq:prediction}, we additionally concatenate $5$-dimensional index embedding to the feature $t_{i,j}\in\mathcal{F}$ to better estimate the global transformation from local transformation features.
While $S$ is another two-layer MLP with $64$ hidden ReLU activations, its output is a scalar without non-linearity; 
this is due to the application of softmax normalization outside $S$.
Note that we do not use the index embedding to avoid strong biases of attentions on certain regions.
Since $G$ and $S$ are applied to all feature vectors across the spatial dimensions, we implement them by multiple $1\times1$ convolutions with batch normalizations.

\subsubsection{Network training}
We build two of the proposed networks with different parametric global transformations: affine and thin-plate spline (TPS) transformations.
To train the network, we adapt the average transformed grid distance loss proposed in~\cite{rocco2017convolutional}, which indirectly measures the distance from the predicted transformation parameters $\theta$ to the ground-truth transformation parameters $\theta_\mathrm{GT}$.
Given $\theta$ and $\theta_\mathrm{GT}$, the transformed grid distance $\mathrm{TGD}(\theta, \theta_\mathrm{GT})$ is obtained by
\begin{equation}
    \mathrm{TGD}(\theta, \theta_\mathrm{GT}) = \frac{1}{|\mathcal{G}|}\sum_{g \in \mathcal{G}}{d\left(\mathcal{T}_\theta\left(g\right), \mathcal{T}_{\theta_\mathrm{GT}}\left(g\right)\right)^2}
\end{equation}
where $\mathcal{G}$ is a set of points in a regular grid, $\mathcal{T}_\theta$ is the transformation parameterized by $\theta$ and $d(\cdot)$ is a distance measure.
We minimize the average TGD of training examples to train the network.
Since every operation within the proposed network is differentiable, the network is trainable end-to-end using a gradient-based optimization algorithm.
We use ADAM~\cite{kingma2014adam} with initial learning rate of $2 \times 10^{-4}$ and batch size of $32$ for $50$ epochs.
During training, the pretrained feature extractor is fixed and only the other parts of the network are finetuned.


==> ECCV 2018 (SA) Camera Ready/sections/offset_kernels.tex <==
% !TEX root = ../nips_2017.tex

%%%%%%%%% BODY TEXT
\section{Offset-Aware Correlation Kernels}
\label{sec:offset_kernels}


During the attention process, each local transformation feature $t_{i,j}$ is fed to two different functions $G$ and $S$ in Eq.~\eqref{eq:attention} and \eqref{eq:att_prob} for the feature projection and the attention score estimation, respectively.
Because the same functions are applied to every local feature across the spatial dimensions, feature representation should be appropriate for translation invariant operations like convolution by encoding local transformations in their feature representation.
To achieve this, we propose offset-aware correlation (OAC) kernels that encode local transformations in a self-contained manner.
The proposed kernels are applied to correlations between source and target features where the kernel weights are shared based on the offsets between these features.
%
%We propose a novel offset-based correlation kernels that are applied to the correlations between features from two input images.
%The proposed method learns multiple kernels of which a weight is shared for all correlations between features with the same offset.
Since each kernel is aligned to the correlations based on the relative offsets, those kernels are able to capture local transformations at each spatial location.
% In this section, we briefly introduce a similar technique called the correlation layer introduced in~\cite{rocco2017convolutional} with its limitation.
% Then, we describe the offset-based correlation kernels that overcome the limitation of the method.
In this section, we briefly describe the correlation layer introduced in~\cite{rocco2017convolutional} with its limitations and explain our approach which is formally interpreted as the proposed OAC kernels.



\subsection{Correlation Layer}
Motivated by classical methods, Rocco~\etal~\cite{rocco2017convolutional} introduce the correlation layer computing correlations of all paired features from the source and target images.
Formally speaking, let $\bm{f}^\mathrm{src}, \bm{f}^\mathrm{trg} \in \mathbbm{R}^{D\times H\times W}$ be feature maps of the source and target images where $H$ and $W$ are the spatial width and height, and $D$ is the number of channels of the feature maps.
The correlation layer takes as inputs the source and target feature maps and constructs a correlation map $\bm{c} \in \mathbbm{R}^{HW \times H \times W}$ by
%
\begin{equation}
    c_{i,j} = {f^\mathrm{src}_{i,j}}^\top \hat{\bm{f}}^\mathrm{trg}
\end{equation}
%
where $c_{i,j} \in \bm{c}$ is a $HW$ dimensional correlation vector at a spatial location $(i, j)$, $f_{i,j}^\mathrm{src} \in \bm{f}^\mathrm{src}$ is a feature vector at a location $(i, j)$, and $\hat{\bm{f}}^\mathrm{trg} \in \mathbbm{R}^{D\times HW}$ is a spatially flattened feature map of $\bm{f}^\mathrm{trg}$.
Note that each correlation vector $c_{i,j}$ contains correlations between a single feature $f_{i,j}^\mathrm{src}$ and all features of $\bm{f}^\mathrm{trg}$, and encodes local transformation of $f_{i,j}^\mathrm{src}$ in the target feature map.
%In~\cite{rocco2017convolutional}, the constructed correlation map is then fed to a convolutional neural network after normalization to regress transformation parameters for geometric matching. 
Note that the values in correlation vectors are arranged by the absolute indices of the target features;
we need the index of the source feature to understand the local transformation of that source feature in the target feature map.

For example, the meaning of a correlation vector $c_{i,j}=[1, 0, 0, 0]^\top$ changes depending on the choice of $(i,j)$ where $H=W=2$ and each element of the vector is the correlation of $f^\mathrm{src}_{i,j}$ with $f^\mathrm{trg}_{0,0}$, $f^\mathrm{trg}_{0,1}$, $f^\mathrm{trg}_{1,0}$ and $f^\mathrm{trg}_{1,1}$.
If $(i,j)=(0,0)$, then meaning of the vector is that the source feature $f^\mathrm{src}_{0,0}$ remains at the location $(0,0)$ in the target feature map.
If $(i,j)=(0,1)$, it means the source feature $f^\mathrm{src}_{0,1}$ moves to the left of its original location in the target feature map.
%
This is especially problematic when applying the attention processes because we apply translation invariant functions, $G$ and $S$, to every local transformation feature where the feature alone should convey sufficient information for estimating the attention scores and generating feature vector for transformation estimation.



\subsection{Reordering correlations and feature compression}
To overcome such limitation, we reorder the correlations of the correlation map using the offsets between source and target features instead of the absolute index of target features.
That is, the correlations with the same relative displacements are arranged in the same channel of the feature map.
This reordering results in $(2H-1)(2W-1)$ possible offsets and thus the output tensor is the size of $(2H-1)(2W-1) \times H \times W$ where many of the values are zeros due to non-existing pairs for some offsets.
To reduce the number of channels, we apply $1\times1$ convolution operation compressing features into a dense representation.

Note that this reordering scheme injects the relative displacement information of an image feature into the correlation vector representation by arranging the dimensions.
Thus, this reordered correlation vector itself already contains local transformation information, and is appropriate as an input to translation invariant operations such as $G$ and $S$ in the attention process.
%Moreover, it is appropriate as an input to translation-invariant operations since an output feature at each location is self-contained in encoding local transformations within the region.

\subsection{Offset-based Correlation Kernels}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.49\linewidth}
\centering
\includegraphics[width=0.7\linewidth]{figures/correlation_kernels_0.pdf}
\subcaption{kernel alignment for $h_{0,0}$}
\label{fig:kernels_00}
\end{subfigure}
%
\begin{subfigure}[b]{0.49\linewidth}
\centering
\includegraphics[width=0.7\linewidth]{figures/correlation_kernels_1.pdf}
\subcaption{kernel alignment for $h_{0,1}$}
\label{fig:kernels_01}
\end{subfigure}
\caption{
Illustration of offset-aware correlation kernel applications at different source locations: (a) at $(0,0)$ and (b) at $(0,1)$.
%Each weight $w_{i,j}$ is associated with a correlation of which source and target features are connected by dotted line.
Each dotted line connects source and target features to compute correlation, and $w_{i,j}$ represents a kernel weight for the dotted line.
Note that kernel weights are associated with different correlation pairs when source locations vary.
%In (a), $\theta_{0,0}$ is associated with the correlation
}
\label{fig:kernels}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We interpret the above reordering schemes with feature compression as a new type of kernels, referred to as OAC kernels, that take two image feature maps and produce a single output feature map containing local transformation features.
%
%The proposed OBC kernels takes as inputs two image feature maps extracted from the source and target images and produces a single output feature map whose feature vector at a spatial location captures the local transformation of the source feature at the same location in the target feature map.
%Local transformation encoding is achieved by using correlations of a source feature at a single location with all target features along the spatial dimensions as the proposed kernels assign weights to each of these correlations.
Note that the weights of $1\times1$ convolution layer are aligned with the reordered correlations.
That is, the weights are shared among those correlation values that are computed from the source and target features with the same offset.

%Formally speaking, let $\bm{f}^\mathrm{src}, \bm{f}^\mathrm{trg} \in \mathbbm{R}^{D\times H\times W}$ be the source and target feature maps respectively where both feature maps are extracted by the same CNN from the source and target images.
Therefore, we formally define a OAC kernel that computes a dense local transformation feature $h^{(n)}_{i,j}$ by
%
\begin{align}
    h_{i, j}^{(n)} &=\sum_{k=1}^{H}{\sum_{l=1}^{W}{w_{i-k, j-l}^{(n)} c_{i,j;k,l}}} \\
    &=\sum_{k=1}^{H}{\sum_{l=1}^{W}{w_{i-k, j-l}^{(n)} {f^\mathrm{src}_{i,j}}^\top f^\mathrm{trg}_{k,l}}}
\end{align}
%
where $c_{i,j;k,l}$ is the correlation between a source feature $f^\mathrm{src}_{i,j}$ and a target feature $f^\mathrm{trg}_{k,l}$, $n$ is the kernel index, and $\Phi^{(n)}= \{w^{(n)}_{s,t}\}$ is a set of the kernel weights.
Each spatial location of the kernel output $\bm{h} \in \mathbbm{R}^{N\times H\times W}$ corresponds to the same location of the source feature map $\bm{f}^\mathrm{src}$.
Note that the kernel weights are indexed by the relative offset between the source and target features, and shared for the target features with the same relative offsets across all spatial locations in the source feature map.
For example, in Fig.~\ref{fig:kernels_00}, $w_{0,0}$ is associated with the target feature at $(0,0)$ because the source location is $(0,0)$.
Also, the same weight $w_{0,0}$ is associated with the target feature at $(0,1)$ when the source location is $(0,1)$ as in Fig.~\ref{fig:kernels_01}.
%In consequence, two outputs of the proposed kernels $h_{i,j}, h_{k,l} \in \mathbbm{R}^{N}$ may differ even when $f_{i,j}^\mathrm{src}=f_{k,l}^\mathrm{src}$ if $(i,j)\ne (k,l)$.
%This weight sharing scheme lets the kernel output capture the spatial relationships between source and target images and encode the local transformations from the source to the target image.

This interpretation allows us to reduce the time complexity of the kernel output computation.
The reordered correlation map with a $1\times1$ convolution requires $N(2H^2-H)(2W^2-W)$ multiplications whereas only $NH^2W^2$ multiplications are required using OAC kernels.



==> ECCV 2018 (SA) Camera Ready/sections/related_work.tex <==
% !TEX root = ../main.tex

%%%%%%%%% BODY TEXT
\section{Related Work}
\label{sec:rel_work}


Most approaches to semantic correspondence are based on dense matching of local image features. 
Early methods extract local features of patches using hand-crafted feature descriptors~\cite{yang2014daisy} such as SIFT~\cite{kim2013deformable,liu2016sift,hur2015generalized,bristow2015dense} and HOG~\cite{ham2016proposal,berg2005shape,taniai2016joint,yang2017object}.
In spite of some success, the lack of high-level semantics in the feature representation makes the approaches suffer from non-rigid deformation and large appearance changes of objects.
While such challenges have been mainly investigated in the area of graph-based image matching~\cite{berg2005shape,cho2010reweighted,duchenne2011graph,cho2013learning}, recent methods~\cite{ufer2017deep,kim2017dctm,kim2017fcss,novotny2017anchornet,zagoruyko2015learning,zbontar2015computing,han2015matchnet,long2014convnets,zhou2016learning,kanazawa2016warpnet} rely on deep neural networks to extract high-level features of patches for robust matching.
More recently, Han \etal~\cite{han2017scnet} propose a deep neural network that learns both a feature extractor and a matching model for semantic correspondence. % with a semantic alignment dataset.
In spite of these developments, all these approaches detect correspondences by matching patches or region proposals based on their local features. In contrast, %our method predicts dense correspondences by global transformation estimation where the entire image is transformed by the predicted transformation parameters.
Rocco \etal~\cite{rocco2017convolutional} propose a global transformation estimation method that is the most relevant work to ours. Their model in \cite{rocco2017convolutional} predicts the transformation parameters from a correlation map obtained by computing correlations of every pair of features in source and target feature maps.
Although this model is similar to ours in that it estimates the global transformation based on correlations of feature pairs, our model is distinguished by the attention process suppressing irrelevant features and the use of the OAC kernels constructing local transformation features.
%
%Although it uses all correlations of every possible feature combination, the correlations themselves do not contain any spatial information and fail to capture local transformations.
%In contrast, the proposed model replaces the correlation layer with offset-based correlation kernels that encodes the spatial relationships in addition to the correlations between features and captures local transformations.
%Since the kernel activations at each spatial location are self-sufficient without extra support for spatial information, these are appropriate for translation-invariant operations such as convolutions, which are used as the subsequent layer in our architecture.

There are some related studies on other tasks using feature correlations such as optical flow estimation~\cite{dosovitskiy2015flownet} and stereo matching~\cite{zbontar2016stereo,luo2016efficient}.
Dosovitskiy \etal\cite{dosovitskiy2015flownet} use correlations between features of two video frames to estimate optical flow, while Zbontar \etal\cite{zbontar2016stereo} and Luo \etal\cite{luo2016efficient} extract feature correlations from patches of images for stereo matching.
Although all these methods utilize the correlations, they extract correlations from features in a limited set of candidate regions.
Moreover, unlike ours, they do not explore the attentive process and the offset-based correlation kernels.

Lately, attention models have been widely explored for various tasks with multi-modal inputs such as image captioning~\cite{xu2015show,mun2017text}, visual question answering~\cite{xu2016ask,yang2016stacked}, attribute prediction~\cite{seo2016progressive} and machine translation~\cite{bahdanau2015neural,luong2015effective}.
In these studies, models attend to the relevant regions referred and guided by another modality such as language, while the proposed model attends based on a self-guidance.
Noh \etal~\cite{noh2017large} use an attention process for image retrieval to extract deep local features, where the attention is obtained from the features themselves as in our work.
%However, the attended features are used for image retrieval in \cite{noh2017large} and is very different from our task.

%To the best of our knowledge, our work is the first in proposing an attention mechanism for the problem of semantic correspondence.




==> sections/attention.tex <==
% !TEX root = ../nips_2017.tex

%%%%%%%%% BODY TEXT


\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/attention.pdf}
    \caption{
    Illustration of attention process. 
    Noisy features in local transformation feature map are filtered by assigning lower probabilities to these locations.
    Arrows in boxes of local transformation feature map demonstrate features encoding local transformations, and grayscale colors in attention distribution represent magnitudes of probabilities where brighter colors mean higher probabilities.}
    \label{fig:att}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi


\section{Attentive Semantic Alignment}
\label{sec:attentive_matching}
We propose an attentive semantic alignment algorithm based on spatial attention.
To this end, we estimate a global transformation between two images, which is given by a linear combination of local transformations.
This section describes how the global transformation is obtained from local transformations by exploiting an attention model while we reserve detailed discussion about the local transformation to Section~\ref{sec:offset_kernels}.
%The local transformations are obtained by computing feature correlation between all pairs of locations in the feature maps extracted from two images. 

%facilitates attention process and focus on reliable local features only. 
%We estimate global transformation by extracting an attended feature and filtering distractors out.
%as illustrated in Fig.~\ref{fig:att}.
%While the matching task involves two input images, 
%The attention process in our model takes a local transformation feature map summarizing the feature relationships between two images, which is described in more details in Section~\ref{sec:offset_kernels}.

%In this section, we first present the overall estimation procedure with the attentive process given a feature map of local transformations, whose construction will be described in Section~\ref{sec:offset_kernels}.

\subsection{Spatial Attention on Local Transformation Features}
\label{sub:att}
Suppose that we have a local transformation feature map $\mathcal{F} \in \mathbbm{R}^{\hat{D}\times\hat{H}\times\hat{W}}$ with $\hat{H}\times\hat{W}$ spatial resolution;
each feature vector $t_{i,j}\in \mathbbm{R}^{\hat{D}}$ encodes the transformation of a local region at $(i,j)$ from a source image to a target image.
Although a feature map $\mathcal{F}$ gives sufficient information to predict the global transformation from a source to a target, local transformation features extracted from a real image pair is noisy due to various reasons such as background clutter and intra-class variations.
Therefore, we propose a model that suppresses unreliable features by the attention process and extracts an attended feature vector that summarizes local transformations from all reliable locations to estimate a accurate global transformation.
In other words, the model computes an attended transformation feature $\tau^\mathrm{att}$ by
%
\begin{align}
    \tau^\mathrm{att} %= %\sum_{i=1}^{\hat{H}}{\sum_{j=1}^{\hat{W}}{\alpha_{i,j}\tau_{i, j}}} 
    = \sum_{i=1}^{\hat{H}}{\sum_{j=1}^{\hat{W}}{\alpha_{i,j}G(t_{i, j})}}
\label{eq:attention}
\end{align}
%
where $G:\mathbbm{R}^{\hat{D}}\rightarrow \mathbbm{R}^{D'}$ is a projection function of $t_{i,j}$ into a $D'$ dimensional vector space and $\bm{\alpha} = \{\alpha_{i,j}\}$ is an attention probability distribution over feature map.
The model computes the attention probabilities by
%
\begin{equation}
    \alpha_{i,j} = \frac{\exp\left({S(t_{i,j})}\right)}{\sum_{k=1}^{\hat{H}}{\sum_{l=1}^{\hat{W}}{\exp\left({S(t_{k,l})}\right)}}} \label{eq:att_prob}
\end{equation}
%
where $S:\mathbbm{R}^{\hat{D}}\rightarrow\mathbbm{R}$ is an attention score function returning a single scalar given a local transformation feature.
%According to Eq.~\eqref{eq:attention}, the contribution of each feature $t_{i,j}$ to the attended feature $\tau^\mathrm{att}$ depends on its attention probability $\alpha_{i,j}$, which is given by scoring the transformation feature $t_{i,j}$ as specified in Eq.~\eqref{eq:att_prob}.
Note that the model learns capability to rejecting noisy features by assigning low attention scores and reducing their contribution to the attended feature.

Once the attended feature $\tau^\mathrm{att}$ over all local transformations is obtained, we compute the global transformation $\theta \in \mathbbm{R}^Q$ by a simple matrix-vector multiplication as
%the model estimates parameters of the global transformation $\theta$ with a fully-connected layer by
%
\begin{equation}
    \theta = W\tau^\mathrm{att} \label{eq:prediction}
\end{equation}
%
where $W \in \mathbbm{R}^{Q\times{D'}}$ is a weight matrix for the linear projection of the attended feature $\tau^\mathrm{att}$.

In summary, we first local transformation between two images and perform a nonlinear embedding using a projection function $G(\cdot)$.
The embedded vector is weighted by spatial attention to compute an attended feature $\tau^\mathrm{att}$ as shown in Eq.~\eqref{eq:attention}.
The global transformation vector is given by a linear projection of the attended feature parametrized by a matrix as presented in Eq.~\eqref{eq:prediction}.

%\subsection{Desired Properties of Local Transformation Features}


==> sections/offset_kernels.tex <==
% !TEX root = ../nips_2017.tex

%%%%%%%%% BODY TEXT
\section{Offset-Aware Correlation Kernels}
\label{sec:offset_kernels}


During the attention process, each local transformation feature $t_{i,j}$ is fed to two different functions $G$ and $S$ in Eq.~\eqref{eq:attention} and \eqref{eq:att_prob} for the feature projection and the attention score estimation, respectively.
Because the same functions are applied to every local feature across the spatial dimensions, feature representation should be appropriate for translation invariant operations like convolution by encoding local transformations in their feature representation.
To achieve this, we propose offset-aware correlation (OAC) kernels that encode local transformations in a self-contained manner.
The proposed kernels are applied to correlations between source and target features where the kernel weights are shared based on the offsets between these features.
%
%We propose a novel offset-based correlation kernels that are applied to the correlations between features from two input images.
%The proposed method learns multiple kernels of which a weight is shared for all correlations between features with the same offset.
Since each kernel is aligned to the correlations based on the relative offsets, those kernels are able to capture local transformations at each spatial location.
% In this section, we briefly introduce a similar technique called the correlation layer introduced in~\cite{rocco2017convolutional} with its limitation.
% Then, we describe the offset-based correlation kernels that overcome the limitation of the method.
In this section, we briefly describe the correlation layer introduced in~\cite{rocco2017convolutional} with its limitations and explain our approach which is formally interpreted as the proposed OAC kernels.



\subsection{Correlation Layer}
Motivated by classical methods, Rocco~\etal~\cite{rocco2017convolutional} introduce the correlation layer computing correlations of all paired features from the source and target images.
Formally speaking, let $\bm{f}^\mathrm{src}, \bm{f}^\mathrm{trg} \in \mathbbm{R}^{D\times H\times W}$ be feature maps of the source and target images where $H$ and $W$ are the spatial width and height, and $D$ is the number of channels of the feature maps.
The correlation layer takes as inputs the source and target feature maps and constructs a correlation map $\bm{c} \in \mathbbm{R}^{HW \times H \times W}$ by
%
\begin{equation}
    c_{i,j} = {f^\mathrm{src}_{i,j}}^\top \hat{\bm{f}}^\mathrm{trg}
\end{equation}
%
where $c_{i,j} \in \bm{c}$ is a $HW$ dimensional correlation vector at a spatial location $(i, j)$, $f_{i,j}^\mathrm{src} \in \bm{f}^\mathrm{src}$ is a feature vector at a location $(i, j)$, and $\hat{\bm{f}}^\mathrm{trg} \in \mathbbm{R}^{D\times HW}$ is a spatially flattened feature map of $\bm{f}^\mathrm{trg}$.
Note that each correlation vector $c_{i,j}$ contains correlations between a single feature $f_{i,j}^\mathrm{src}$ and all features of $\bm{f}^\mathrm{trg}$, and encodes local transformation of $f_{i,j}^\mathrm{src}$ in the target feature map.
%In~\cite{rocco2017convolutional}, the constructed correlation map is then fed to a convolutional neural network after normalization to regress transformation parameters for geometric matching. 
Note that the values in correlation vectors are arranged by the absolute indices of the target features;
we need the index of the source feature to understand the local transformation of that source feature in the target feature map.

For example, the meaning of a correlation vector $c_{i,j}=[1, 0, 0, 0]^\top$ changes depending on the choice of $(i,j)$ where $H=W=2$ and each element of the vector is the correlation of $f^\mathrm{src}_{i,j}$ with $f^\mathrm{trg}_{0,0}$, $f^\mathrm{trg}_{0,1}$, $f^\mathrm{trg}_{1,0}$ and $f^\mathrm{trg}_{1,1}$.
If $(i,j)=(0,0)$, then meaning of the vector is that the source feature $f^\mathrm{src}_{0,0}$ remains at the location $(0,0)$ in the target feature map.
If $(i,j)=(0,1)$, it means the source feature $f^\mathrm{src}_{0,1}$ moves to the left of its original location in the target feature map.
%
This is especially problematic when applying the attention processes because we apply translation invariant functions, $G$ and $S$, to every local transformation feature where the feature alone should convey sufficient information for estimating the attention scores and generating feature vector for transformation estimation.



\subsection{Reordering correlations and feature compression}
To overcome such limitation, we reorder the correlations of the correlation map using the offsets between source and target features instead of the absolute index of target features.
That is, the correlations with the same relative displacements are arranged in the same channel of the feature map.
This reordering results in $(2H-1)(2W-1)$ possible offsets and thus the output tensor is the size of $(2H-1)(2W-1) \times H \times W$ where many of the values are zeros due to non-existing pairs for some offsets.
To reduce the number of channels, we apply $1\times1$ convolution operation compressing features into a dense representation.

Note that this reordering scheme injects the relative displacement information of an image feature into the correlation vector representation by arranging the dimensions.
Thus, this reordered correlation vector itself already contains local transformation information, and is appropriate as an input to translation invariant operations such as $G$ and $S$ in the attention process.
%Moreover, it is appropriate as an input to translation-invariant operations since an output feature at each location is self-contained in encoding local transformations within the region.

\subsection{Offset-based Correlation Kernels}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.49\linewidth}
\centering
\includegraphics[width=0.7\linewidth]{figures/correlation_kernels_0.pdf}
\subcaption{kernel alignment for $h_{0,0}$}
\label{fig:kernels_00}
\end{subfigure}
%
\begin{subfigure}[b]{0.49\linewidth}
\centering
\includegraphics[width=0.7\linewidth]{figures/correlation_kernels_1.pdf}
\subcaption{kernel alignment for $h_{0,1}$}
\label{fig:kernels_01}
\end{subfigure}
\caption{
Illustration of offset-aware correlation kernel applications at different source locations: (a) at $(0,0)$ and (b) at $(0,1)$.
%Each weight $w_{i,j}$ is associated with a correlation of which source and target features are connected by dotted line.
Each dotted line connects source and target features to compute correlation, and $w_{i,j}$ represents a kernel weight for the dotted line.
Note that kernel weights are associated with different correlation pairs when source locations vary.
%In (a), $\theta_{0,0}$ is associated with the correlation
}
\label{fig:kernels}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We interpret the above reordering schemes with feature compression as a new type of kernels, referred to as OAC kernels, that take two image feature maps and produce a single output feature map containing local transformation features.
%
%The proposed OBC kernels takes as inputs two image feature maps extracted from the source and target images and produces a single output feature map whose feature vector at a spatial location captures the local transformation of the source feature at the same location in the target feature map.
%Local transformation encoding is achieved by using correlations of a source feature at a single location with all target features along the spatial dimensions as the proposed kernels assign weights to each of these correlations.
Note that the weights of $1\times1$ convolution layer are aligned with the reordered correlations.
That is, the weights are shared among those correlation values that are computed from the source and target features with the same offset.

%Formally speaking, let $\bm{f}^\mathrm{src}, \bm{f}^\mathrm{trg} \in \mathbbm{R}^{D\times H\times W}$ be the source and target feature maps respectively where both feature maps are extracted by the same CNN from the source and target images.
Therefore, we formally define a OAC kernel that computes a dense local transformation feature $h^{(n)}_{i,j}$ by
%
\begin{align}
    h_{i, j}^{(n)} &=\sum_{k=1}^{H}{\sum_{l=1}^{W}{w_{i-k, j-l}^{(n)} c_{i,j;k,l}}} \\
    &=\sum_{k=1}^{H}{\sum_{l=1}^{W}{w_{i-k, j-l}^{(n)} {f^\mathrm{src}_{i,j}}^\top f^\mathrm{trg}_{k,l}}}
\end{align}
%
where $c_{i,j;k,l}$ is the correlation between a source feature $f^\mathrm{src}_{i,j}$ and a target feature $f^\mathrm{trg}_{k,l}$, $n$ is the kernel index, and $\Phi^{(n)}= \{w^{(n)}_{s,t}\}$ is a set of the kernel weights.
Each spatial location of the kernel output $\bm{h} \in \mathbbm{R}^{N\times H\times W}$ corresponds to the same location of the source feature map $\bm{f}^\mathrm{src}$.
Note that the kernel weights are indexed by the relative offset between the source and target features, and shared for the target features with the same relative offsets across all spatial locations in the source feature map.
For example, in Fig.~\ref{fig:kernels_00}, $w_{0,0}$ is associated with the target feature at $(0,0)$ because the source location is $(0,0)$.
Also, the same weight $w_{0,0}$ is associated with the target feature at $(0,1)$ when the source location is $(0,1)$ as in Fig.~\ref{fig:kernels_01}.
%In consequence, two outputs of the proposed kernels $h_{i,j}, h_{k,l} \in \mathbbm{R}^{N}$ may differ even when $f_{i,j}^\mathrm{src}=f_{k,l}^\mathrm{src}$ if $(i,j)\ne (k,l)$.
%This weight sharing scheme lets the kernel output capture the spatial relationships between source and target images and encode the local transformations from the source to the target image.

This interpretation allows us to reduce the time complexity of the kernel output computation.
The reordered correlation map with a $1\times1$ convolution requires $N(2H^2-H)(2W^2-W)$ multiplications whereas only $NH^2W^2$ multiplications are required using OAC kernels.


